On Integrated Sensing and Communication Waveforms with Tunable PAPR

We present a novel approach to the problem of dual-functional radar and communication (DFRC) waveform design with adjustable peak-to-average power ratio (PAPR), while minimizing the multi-user communication interference and maintaining a similarity constraint towards a radar chirp signal. The approach is applicable to generic radar chirp signals and for different constellation sizes. We formulate the waveform design problem as a non convex optimization problem. As a solution, we adopt the alternating direction method of multipliers (ADMM), hence iterating towards a stable waveform for both radar and communication purposes. Additionally, we prove convergence of the proposed method and analyze its computational complexity. Moreover, we offer an extended version of the method to cope with imperfect channel state information (CSI). Finally, we demonstrate its superior performance through simulations, in comparison to state-of-the-art radar-communication waveform designs.

==> actions01/grammar-typos.tex <==
\color{darkgreen}
\begin{itemize}
	\item In the first paragraph of the Introduction, "the study" has been replaced by \textcolor{blue}{research}.
	\item The following sentence in the Introduction "Thanks to such approach, this naturally accomplishes full collaboration between radar and communication sub-systems, while only requiring one smaller-size, lower-cost, and lower-complexity platform" contains some typos and has been replaced as "Thanks to such \textcolor{blue}{an} approach, full collaboration between radar and communication sub-systems \textcolor{blue}{can be accomplished}, while only requiring  smaller-size, lower-cost, and \textcolor{blue}{less-complex platforms}"
	\item In the Introduction, "the \ac{MIMO}" has been replaced by "\textcolor{blue}{\ac{MIMO}}".
	\item In the Introduction, "high power amplifier (HPA)" has been replaced with \textcolor{blue}{"high power amplifiers (HPAs)"}.
	\item In the Introduction, "and a lower \ac{PAPR} is favored in many applications utilizing \acp{HPA} as part of their transmit chains." has been replaced by "\textcolor{blue}{In principle, low \ac{PAPR} waveforms are desired, as it enables us to tune the \ac{HPA}'s Q-point as close as possible towards the optimal operating point, with no risk of clipping.}"
	\item In the Introduction, "while sacrificing the" has been replaced by "\textcolor{blue}{at the price of increased}"
	\item In the Introduction, we have ommited "of the utilized constellation".
	\item In the Introduction, "baseband pre-distortions" has been replaced by "\textcolor{blue}{baseband pre-distortion methods}"
	\item In Section \ref{subsec:contributions}, the following sentence "This paper considers DFRC waveform design towards communication users, while listening to received echo of the transmitted signal," has been replaced by "This paper considers \ac{DFRC} \textcolor{blue}{\ac{BS}} waveform design \textcolor{blue}{with tunable \ac{PAPR}, intended for \ac{DL}} communication users, while listening to \textcolor{blue}{the} received echo of the transmitted signal."
	\item In Section \ref{subsec:comm-sys-model}, the following sentence: ".. in the \ac{DL} sense, from a \ac{DFRC} \ac{BS}.." is now ".. in the \ac{DL} sense, \textcolor{blue}{initiated} from a \ac{DFRC}\ac{BS}.."
	\item In Section \ref{sec:framework}, "be easily noted" is replaced with "be easily \textcolor{blue}{verified}".
	\item Just below equation \eqref{eq:update-alpha-problem}, "ommiting" is replaced with \textcolor{blue}{omitting}.
	\item In Section \ref{sec:admm}, we have re-written the text just below equation \eqref{eq:beta-update} as follows, \\
\textcolor{blue}{\input{actions01/text-below-beta.tex}}
	
\end{itemize}



Also, we have corrected the following typos within equations:
\begin{itemize}
	\item We have corrected $\pmb{x}_{\comm}$ in \eqref{eq:gradient-at-x-expanded} to become \textcolor{blue}{$\bar{\pmb{x}}_{\comm}$}. The corresponding equation is now
\begin{equation*}
\begin{split}
	2( \pmb{x}^{(m+1)} &- \textcolor{blue}{\bar{\pmb{x}}_{\comm}} ) + \pmb{u}^{(m)} + \pmb{v}^{(m)} + \sum\limits_{n=1}^{NL} \bar{\pmb{F}}_n^T \pmb{w}_n^{(m)} \\
	&+ \rho (\bar{\pmb{x}}^{(m+1)} - \pmb{\alpha}^{(m)}) 
	+ \rho(  \bar{\pmb{x}}^{(m+1)} - \bar{\pmb{x}}_0 - \pmb{\beta}^{(m)} )\\
	&+ \rho \sum\limits_{n=1}^{NL} \bar{\pmb{F}}_n^T(\bar{\pmb{F}}_n \bar{\pmb{x}}^{(m+1)} - \pmb{\gamma}_n^{(m)})  = \pmb{0}.
\end{split}
\end{equation*}	
	
	
	
	\item  We have corrected the notation \textcolor{blue}{$\bar{\pmb{x}}^{(m+1)}$} instead of ${\pmb{x}}^{(m+1)}$ in the first line of the main loop of Algorithm 1. 
	\item We have replaced  $\bar{\pmb{x}}^{(M_{{iter}})}$ with \textcolor{blue}{$\bar{\pmb{x}}^{(M_{{iter}})}$} in the last line of Algorithm 1.
%	\item Below equation \ref{eq:beta-update}, "except $\gamma_n$" is now "except \textcolor{blue}{$\pmb{\gamma}_n$}"
	\item Likewise, as in the previous item, we replace $\gamma_n$ in the constraint of equation \eqref{eq:update-gamma-problem-equivalent} with \textcolor{blue}{$\pmb{\gamma}_n$}.
	\item In equation \eqref{eq:gradient-at-x-expanded}, $\pmb{x}^{(m+1)}$ is replaced with \textcolor{blue}{$\bar{\pmb{x}}^{(m+1)}$}.
	\item Just on top of equation \eqref{eq:x-update}, $\pmb{x}^{(m+1)}$ is replaced with \textcolor{blue}{$\bar{\pmb{x}}^{(m+1)}$}.
	\item In equation \eqref{eq:augmented-lag-multiplier-all}, the argument of the augmented Lagrangian function should take all $\pmb{\gamma}_1 \ldots \pmb{\gamma}_{NL}$ instead of $\pmb{\gamma}_n$. Likewise, the augmented Lagrangian function should take all $\pmb{w}_1 \ldots \pmb{w}_{NL}$ instead of $\pmb{w}_n$. For this, we now denote $\mathcal{L}_{\rho}(\bar{\pmb{x}},\pmb{\alpha},\pmb{\beta},\textcolor{blue}{\pmb{\gamma}},\pmb{u},\pmb{v},\textcolor{blue}{\pmb{w}}) $ instead of the missing $\mathcal{L}_{\rho}(\bar{\pmb{x}},\pmb{\alpha},\pmb{\beta},\pmb{\gamma}_n,\pmb{u},\pmb{v},\pmb{w}_n)$ then define $\textcolor{blue}{\pmb{w}}, \textcolor{blue}{\pmb{\gamma}} $ below equation \eqref{eq:augmented-lag-multiplier-all} as follows: \textcolor{blue}{$\pmb{\gamma} = \begin{bmatrix} \pmb{\gamma}_1^T  \ldots \pmb{\gamma}_{NL}^T \end{bmatrix}^T $, $\pmb{w} = \begin{bmatrix} \pmb{w}_1^T  \ldots \pmb{w}_{NL}^T \end{bmatrix}^T $}. Now, equation \eqref{eq:augmented-lag-multiplier-all} is given as 
	\textcolor{blue}{\input{actions01/admm-round-robin-equations.tex}}
	
	The above change also applies to equations \eqref{eq:first-opt}, \eqref{eq:gradient-at-x}, \eqref{eq:second-opt}, the cost in equation \eqref{eq:update-alpha-problem}, equation \eqref{eq:third-opt}, the cost in equation \eqref{eq:update-beta-problem}, equation \eqref{eq:fourth-opt}
	
	\item Equation \eqref{eq:update-gamma-problem-equivalent} should be for $NL$ optimization problems. We have now clarified this by adding on top of equation \eqref{eq:update-gamma-problem-equivalent}: \textcolor{blue}{$NL$ independent optimization problems} and below this equation \eqref{eq:update-gamma-problem-equivalent}, \textcolor{blue}{for $n = 1\ldots NL$.} 
	
	\item Equation \eqref{eq:w-update} should be for all $n$. This has been added.
\end{itemize}






%% Replaced sentences (not typos, not grammar)
Additionally, the following sentences/phrases/equations have been replaced for better presentation purposes and/or a more concise description:
\begin{itemize}
	\item In the abstract, we have replaced "Additionally, we prove convergence of the proposed iterative waveform design and demonstrate its superior performance by computer simulations, in comparison to state-of-the-art radar-communication waveform designs. " with \textcolor{blue}{Additionally, we prove convergence of the proposed method and analyze its computational complexity. Moreover, we offer an extended version of the method to cope with imperfect channel state information (CSI). Finally, we demonstrate its superior performance through simulations, in comparison to state-of-the-art radar-communication waveform designs.}
	\item In the first paragraph of the introduction, "recognized" has been replaced by \textcolor{blue}{identified}.
	\item  In the Introduction, "For example in \cite{wang2021model} \ac{PAPR} reduction techniques are proposed for OFDM, and in \cite{chafii2016necessary,chafii2014papr}, low \ac{PAPR} waveform design have been studied." has been replaced by "\textcolor{blue}{For instance, the work in \cite{wang2021model} proposes \ac{PAPR} reduction methods for \ac{OFDM} and \cite{chafii2016necessary} derives necessary conditions for waveforms exhibiting a better \ac{PAPR} than \ac{OFDM}.}"
	\item In Section \ref{subsec:contributions}, we have omitted "which is designed for both radar and communication tasks." to avoid repetition, as the previous statement is self-explanatory. 
	\item In Section \ref{subsec:contributions}, the following item has been removed from Insights to avoid repetition "Simulations reveal that the proposed ADMM-based waveform design is always guaranteed to converge to a stable waveform."
	\item Given all the changes made in the manuscript, we have conducted major changes to the first paragraph of Section \ref{subsec:organization}. It is now given as follows:
	 \textcolor{blue}{\input{actions01/organization.tex}}
	 \item We introduced replaced occurrences of "base station" with BS in different parts of the manuscript, most notable in Section \ref{sec:systemmodel} and Section \ref{sec:conclusion}.
	 \item Since equations \eqref{eq:u-update}, \eqref{eq:v-update} and \eqref{eq:w-update} were mentioned as part of equation \eqref{eq:update-ADMM-equations-all}, we have omitted the last three equations of equation \eqref{eq:update-ADMM-equations-all}.
	 \item In Section \ref{subsec:comm-sys-model}, the following statement "is the vector of received signals" is now "is the \textcolor{blue}{matrix} of received signals". This is because $\pmb{Y}_c$ is a matrix and not a vector.
	\item Since we have introduced $E_{\MUI}$ in equation \eqref{eq:EMUI}, we have replaced $\Vert  \pmb{\MUI} \Vert^2_F$ with \textcolor{blue}{$E_{\MUI}$} in equations: \eqref{eq:problem1}, \eqref{eq:problem2} 
	 \item The following text has been omitted since we have not used this property: "Moreover, one way of minimizing the total multi-user interference is to minimize the total sum of $\MUI_k$, i.e. $\sum\limits_{k=1}^K  \Vert  \pmb{\MUI}_k \Vert^2_F $. Furthermore, using the separability property of $\MUI$ over communication users, we have 
\begin{equation}
	\Vert  \pmb{\MUI} \Vert^2_F
	=
	\sum\limits_{k=1}^K  \Vert  \pmb{\MUI}_k \Vert^2_F,
\end{equation} " 
	\item We have re-written equation \eqref{eq:final-problem-equivalent-nonaugmented} to gain more space.
	\item The following text has been removed to accommodate more space for literature review "It is worth noting that \ac{ADMM} is an iterative algorithm initially intended for solving convex optimization problems through parallelization, and found applications in different fields, such as multi-agent optimization \cite{chang2014multi} and graph signal processing \cite{chan2019performance}, just to name a few."
	\item To compress equation \eqref{eq:update-ADMM-equations-all}, we have introduced a new notation, defined in the notations section that is: \textcolor{blue}{For two vectors, $\pmb{x}$ and $\pmb{y}$ $\begin{bmatrix}
		\pmb{x} , \pmb{y}
	\end{bmatrix}^{(m)}$ denotes $\begin{bmatrix}
		\pmb{x}^{(m)} , \pmb{y}^{(m)}
	\end{bmatrix}$ }. 
\end{itemize}

















==> actions01/summary-of-actions.tex <==
In light of the reviewers comments, we summarize our action items as follows:
\begin{itemize}
	\item We have not only included the problem formulation under imperfect CSI, considering the norm-bounded case; but we have also added a Section (Section \ref{sec:imperfect-CSI}) to reformulate and solve the problem under imperfect CSI. As a result, we offer an extended version of our Algorithm tailored for the imperfect CSI case.
	\item We have added an extra Section (Section \ref{sec:complexity}) to conduct complexity analysis of the proposed method. At the end of the section, we have compared it with the complexity of state-of-the-art methods.
	\item We have added a new Section (Section \ref{sec:impact}) in order to clarify how the PAPR can impact the performance of sensing (chirp similarity) or communications (MUI) especially when considering HPA in real transmitting chains.
	\item The literature review is now investigated in depth as more references have been accommodated. As a result, many related work have been included.
	\item We have included the motivation behind using time samples for DFRC signals.
	\item We have now explained the number of time samples taken in the simulation section, as well as the effect of different constellations on each figure.
	\item We have now improved the quality of presentation of the paper, through proof-reading, correcting typos and grammar errors, re-writing many statements, improving equation alignments, removing "F" as subscript of Frobenius norm when it is not used, rearranged notation definitions appropriately. 
	\item We have now presented a more direct or detailed description of DFRC dedicated for B5G/6G scenarios in mMTC/URLLC/eMBB in Section \ref{sec:introduction}.
	\item We have defined the acronym CCDF.
	\item In the simulations section (first paragraph), we have made clear what $L$ is and the radar waveform that is used for similarity.
	\item The formulations and equations in the manuscript have been revised and we have corrected all misconceptions, ambiguities and equation typos.
	\item The format of the paper has been revised, and the the algorithm and references now follow the IEEE format.
	\item We also provided some references that under a unit energy constellation, maximizing SINR is equivalent of minimizing MUI.
	\item In the radar system model, the array steering vectors and their dimensions are now explained.
	\item We have clarified in what sense the QCQP convex bound is a lower bound.
	\item We have clarified what created the difference between the methods in Fig. 7 (in the first submission) when $\epsilon$ is all the same.
	\item We have taken the average of all simulations to plot Fig. 3. and Fig. 5 (in the first submission). These figures correspond to Fig. \ref{fig:CostvsIter_response} and Fig. \ref{fig:PAPRvsIter_response} in this response letter, respectively.
	\item We have improved the resolution of Fig. 9 (in the first submission).
	\item We have compared with reference [30] (in the first submission -  reference \cite{hu2022low} in this response letter) in simulations and revealed more insights accordingly. 
	\item We have now unified the units of the variable $\eta$ in Fig. 3 (in the first submission) and Fig. 5 (in the first submission).
	\item We have added a paragraph in sub-Section \ref{subsec:sim-papr-behaviour} to give more explanation about Fig. 5 (in the first submission).
	\item We have clarified why the capacity maximization problem is different, i.e. why our paper considers minimization of the Euclidean norm of the difference zero-forcing preceded signal and the transmitted signal. We have also clarified why the problem also affects the SINR, and hence the capacity.
	\item We have clarified that the convergence analysis has been added here for sake of completeness and we do not claim that the main novelty of our work is in the derivations. But, the novelty is the insight we get from it, and not the derivation itself.
	\item We have made clear how the capacity calculation is done in Fig. 6 (in the first submission). We have also clarified that the MUI affects the SINR even when there is correlation.
	\item We have also made clear that indeed the sum-rate is the summation of all user rates and that average sum rate is the sum-rate divided by the number of users. We have also indicated that the achievable rate bound is a lower bound of the capacity according to \cite{mohammed2013per}.
	\item We have acknowledged all the anonymous reviewers for their constructive comments, which contributed in improving the manuscript.
\end{itemize}





\textbf{Deleted Items:} We have deleted/resized the following items to respect the 15-page double column limit as per the submission guidelines:
\begin{itemize}
	\item Fig.2(c) and Fig.2(d) have been deleted due to lack of space.
	\item Fig. \ref{fig:PulseGainCompression} have been resized.
\end{itemize}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
